Efficient Algorithms for Stochastic Ridepooling Assignment with Mixed Fleets

Ride-pooling, which accommodates multiple passenger requests in a single trip, has the potential to significantly increase fleet utilization in shared mobility platforms. The ride-pooling assignment problem finds optimal co-riders to maximize the total utility or profit on a shareability graph, a hypergraph representing the matching compatibility between available vehicles and pending requests. With mixed fleets due to the introduction of automated or premium vehicles, fleet sizing and relocation decisions should be made before the requests are revealed. Due to the immense size of the underlying shareability graph and demand uncertainty, it is impractical to use exact methods to calculate the optimal trip assignments. Two approximation algorithms for mid-capacity and high-capacity vehicles are proposed in this paper; The respective approximation ratios are $\frac1{p^2}$ and $\frac{e-1}{(2e+o(1)) p \ln p}$, where $p$ is the maximum vehicle capacity plus one. The performance of these algorithms is validated using a mixed autonomy on-demand mobility simulator. These efficient algorithms serve as a stepping stone for a variety of multimodal and multiclass on-demand mobility applications.

==> deleted.tex <==
However, we show a negative result by examining the submodularity of $Q(y, \xi)$.  

For an arbitrary set of hyperedges $A$, we denote a set function $v(A) = \sum_{e\in A} v_e $ and  $v^* =  \max_{A\in \mathcal{I}} v(A)$, respectively.

\begin{remark}
 $v(A)$ is not a submodular function and thus any naive greedy algorithm is arbitrarily bad.
\end{remark}

\proof{Proof:}
Consider a ridehailing system with two drivers and two trip requests in Figure \ref{fig:2}. 
\begin{figure}[!htb]
	\centering
	\includegraphics[width=0.4\textwidth]{figure/fig2.png}
	\caption{A simple counterexample for non-submodular function $v(A)$}
	\label{fig:2}
\end{figure}

Each driver can take at most one trip and the value of each assignment follows $v_1 > v_2 > v_3 > 0$. 
Let $A = \{e_2\}$ and $B = \{e_1, e_2\}$.  
We have
\begin{align*}
0 = v(A + \{e_3\}) - v(A) < v(B+\{e_3\}) - v(B) = v_3.
\end{align*}


Thus, the set function $v(A)$ is not submodular by definition.  \hfill $\square$
\endproof 

Since the second-stage objective function is not submodular in an arbitrary scenario, this work proposes alternative algorithms to tackle the computational issue in SRADS.  
Compared to greedy algorithms for p-extendible systems, obtaining the same approximation ratio with other approaches, e.g.,  local-search  \citep{feldman2011improved,lee2013matroid}, could be much more challenging due to significant effort in customization.



When the algorithm considers to replace vehicle $i_1$ by  vehicle $i_2$, i.e.,  $S_{R'} = S_R \backslash \{i_1\} + \{i_2\}$, the marginal value is  $ U_{i_1 i_2} = \hat{v}(S_{R'}) - \hat{v}(S_R)$.



The marginal value can be decomposed into three parts: 
\begin{enumerate}
	\item $U_{i_1 i_2}^{i_2}$: The increase value from including the hyperedges containing $i_2$;
	\item $U_{i_1 i_2}^{i_1}$:  The decrease value from excluding the hyperedges containing $i_1$;
	\item   $U_{i_1 i_2}^{nb(i_2)} $:  The decrease value from excluding the hyperedges intersecting with demand assigned to $i_2$.
\end{enumerate}

In sum, we have:
\begin{align*}
	U_{i_1 i_2} = U_{i_1 i_2}^{i_2} + U_{i_1 i_2}^{i_1} + U_{i_1 i_2}^{nb(i_2)} 
\end{align*}


 In the non-zero LP-relaxation solution $x_{OPT(i_2)}$ and $x'_{ALG(i_1)}$ for demand $a$, we define new variables $\Delta_{fe}^a$ as in Figure \ref{fig:5}. 
 For example, $\Delta_{f_1 e_1}^a = x_{e_1}$, $\Delta_{f_1 e_2}^{a} = x'_{f_1} - x_{e_1}$, and so forth.  
 We observe that, for arbitrary hyperedges, we have:


Define all demand covered in the LP-relaxation in the scenario $\xi_{\ell} $ as a set $A(i_2)$. 
In each swap subroutine for $S_{R(i_1, i_2)}$, the marginal value is given by
\begin{align}
	U_{i_1 i_2} =& \hat{v}(S_{R'}) - \hat{v}(S_R)  \nonumber \\
	=&  \frac{1}{N} \sum_{\ell \in [N]} \left[ \hat{v}(R(i_2))  - \hat{v}(R(i_1)) - \sum_{a\in A(i_2)} \sum_{f\in ALG(i_1)} \sum_{e\in OPT(i_2)} \Delta_{fe}^a \right]. \label{eq6}
\end{align}

The last term in the parenthesis of eq. \eqref{eq6} can be further reduced as: 
\begin{align*}
	\sum_{a\in A(i_2)} \sum_{f\in ALG(i_1)} \sum_{e\in OPT(i_2)} \Delta_{fe}^a =&  \sum_{f\in ALG(i_1)} \sum_{a\in A(i_2)} \sum_{e\in OPT(i_2)} \Delta_{fe}^a \\
	=&   \sum_{a\in A(i_2)} \sum_{f\in ALG(i_1)} x'_f
	\leq (p-1) \sum_{f\in ALG(i_1)} x'_f
\end{align*}

The last inequality is because the deterministic counterpart of eq.\eqref{alg2} is a p-extendible system, where $p := 1+\max_{i\in S_A\cup S_B} \{C_i\}$ contains one vehicle vertex in $S$.  

Define the mapping from the optimal set $S_{O}$ to the suboptimal selection of augmented supply from the algorithm $S_{R}$ as $\mathcal{M}: S_O\to S_R$. 
%Note that $v(nb(e(i_2^*,*))) = \sum_{e'\in nb(e(i_2^*,\cdot))} v_{e'}$. Since we show SRADS is a p-extendible system in Proposition \ref{prop1}, we have $|nb(e(i_2^*,*) \cap R(\xi_{\ell}) )|\leq p-1$. Define a projection $\mathcal{M}:= S_O\to S_R$ and $(i_2^*, i_1^*)\in \mathcal{M}$.  
We are interested in comparing the distinct subset between $S_{O}$ and $S_{R}$. 
Each swap operation with $i_1^*$ and $i_2^*$ aims to replace a vertice in $S_R$ with a vertice in $S_O$. 
Summing over all the local search iterations, we have:
\begin{align*}
	\sum_{(i_2^*, i_1^*)\in \mathcal{M}} U_{i_1^* i_2^*}  =& \frac{1}{N} \sum_{(i_2^*, i_1^*)\in \mathcal{M}}  \sum_{\ell \in [N]} \left[ \hat{v}(R(i_2))  - \hat{v}(R(i_1)) - \sum_{a\in A(i_2)} \sum_{f\in ALG(i_1)} \sum_{e\in OPT(i_2)} \Delta_{fe}^a \right] \\
	\leq& \frac{1}{N} \sum_{(i_2^*, i_1^*)\in \mathcal{M}}  \sum_{\ell \in [N]} \left[ \hat{v}(R(i_2))  - \hat{v}(R(i_1)) - (p-1) \sum_{f\in ALG(i_1)} x'_f \right]  \\
	\leq& \frac{1}{N} \left[  \sum_{\ell\in[N]} \hat{v}(S_O, \xi_{\ell}) -  p \sum_{\ell \in [N]} \hat{v}(S_R, \xi_{\ell})  \right]  \\
	\leq& 0
\end{align*}


The first inequality is because SRADS in a given scenario is a p-extendible system. 
Each $e(i_2^*, \cdot)$ being added is associated with at most  $p$ hyperedges including the one with $i_1^*$. 
As a result, the rest of hyperedges cannot be eliminated more than $(p-1)$ times. 
The last inequality is due to the stopping criteria of local search algorithm.   
The sample approximation of the optimum value is $v(S_O) = \sum_{\ell \in [N]} v(S_O, \xi_{\ell}))$.    %However, this computation requires solving the p-set packing problem exactly for each $T(\xi)$ given $S_R$, which is not solvable in polynomial time.

Combing the prior results, we use an LP-relaxation  $\hat{v}(S_R, \xi_{\ell})$ over all sampled scenarios $\xi_{\ell}, \ell \in [N]$ so we have:
\begin{align*}
	\sum_{\ell\in[N]} v(S_O, \xi_{\ell}) \leq  \sum_{\ell\in[N]} \hat{v}(S_O, \xi_{\ell})  \leq p \sum_{\ell\in[N]} \hat{v}(S_R, \xi_{\ell}),
\end{align*}
which proves the $\frac{1}{p}$-approximation for the final selection of vehicles in the augmented set.


\begin{equation*}
	\frac{1}{N} \sum_{\ell \in [N]} \hat{v}(S_{R'}, \xi_\ell) \geq
	 \frac{K-p}{N K} \sum_{\ell \in [N]} \hat{v}(S_{R'}, \xi_{\ell}) + \frac{1}{N K } \sum_{\ell\in [N]} \hat{v}(S_O, \xi_{\ell}).
\end{equation*}

By induction, in the $k^{th}$ iteration, the value is given by:
\begin{align*}
\frac{1}{N} \sum_{\ell \in [N]} \hat{v} (S_{R'}, \xi_\ell) 
\geq & \frac{1}{p} \Big[1 - (1 - \frac{p}{K} )^{k} \sum_{\ell\in [N]} \hat{v}(S_O, \xi_\ell) \Big] \\
 \geq &  (\frac{1}{p} -\epsilon) \sum_{\ell\in [N]} \hat{v}(S_O, \xi_\ell)
\end{align*}
where we set $k = \frac{K}{p}\ln (\frac{1}{\epsilon})$. 
This means that the local search conducts at most $\frac{K}{p}\ln (\frac{1}{\epsilon})$ iterations to obtain the $(\frac{1}{p} - \epsilon)$-approximation ratio.


\begin{subequations}  \label{eq7}
	\begin{align}
	\hat{v}(S_R) = &\max_{x: |S_R|\leq K} \frac{1}{N}\sum_{\ell \in [N]}  \sum_{e\in E(\xi_{\ell})} v_e x_e \tag{\ref{eq7}} \\
	s.t. & \sum_{e\in E_{i, \ell} } x_e \leq 1, & \forall i\in V_{\ell } , \forall \ell \in [N]  \\
	& x_e \geq 0, & \forall e \in E_\ell , \forall \ell \in [N]  \\
	& x_e = 0, & \text{ if } e \not\sim S_R \cup S_B 
	\end{align}
\end{subequations}


